CoLAS: Multimodal Corroboration of Latent Asset Signals for Financial Trading

Financial trading relies on extracting reliable signals from heterogeneous market modalities such as price series, breaking news, and investor sentiment. Existing multimodal methods primarily combine heterogeneous modalities to exploit complementarity, treating each modality as equally valuable while overlooking whether different modalities provide mutually supportive evidence for the same trading signal. However, this task-conditioned and non-canceling support, termed multimodal corroboration, is particularly valuable, especially for financial trading. Because individual financial views are noisy and weakly informative, support that persists across heterogeneous views may provide a more stable task-relevant signal than evidence appearing in only one view. To exploit this property, we propose CoLAS (multimodal Corroboration of Latent Asset Signals), a framework that operationalizes multimodal corroboration as a trainable task-conditioned representation for trading prediction. The modality representations are organized into a per-instance matrix, where a softmax-based spectral objective strengthens its dominant shared component. Signed modality contributions then determine whether this component provides non-canceling support and construct the resulting corroborated signal. A coupled robustness-aware consistency objective further preserves the resulting corroborated signal when a modality is corrupted or missing. Extensive experiments on stock and cryptocurrency datasets demonstrate the effectiveness of our proposed CoLAS, yielding consistent improvements in both annualized return and Sharpe ratio over existing methods.

==> tables/RQ4_smp_task.tex <==
\begin{table}[H]
\centering
\caption{ACC and MCC performance of NewsLLM across different stocks.}
\label{tab:acc_mcc_all}
\vspace{-0.2cm}
\scalebox{0.8}{
\begin{threeparttable}
\begin{tabular}{@{}lcccccc@{}}
\toprule
\textbf{Method} & \multicolumn{2}{c}{\textbf{AAPL}} & \multicolumn{2}{c}{\textbf{AMZN}} & \multicolumn{2}{c}{\textbf{GOOG}} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
 & ACC & MCC & ACC & MCC & ACC & MCC \\
\midrule
\texttt{NewsLLM w/o FoE} & 53.02 & 0.0431 & 50.30 & -0.0044 & 52.71 & 0.0533 \\
\texttt{NewsLLM}         & 61.33 & 0.2262 & 59.38 & 0.1914  & 60.94 & 0.1749 \\
Improvement     & 15.67\% & 0.1831 & 18.05\% & 0.1958 & 15.61\% & 0.1216 \\
\midrule
\textbf{Method} & \multicolumn{2}{c}{\textbf{MSFT}} & \multicolumn{2}{c}{\textbf{TSLA}} & \multicolumn{2}{c}{\textbf{Average}} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
 & ACC & MCC & ACC & MCC & ACC & MCC \\
\midrule
\texttt{NewsLLM w/o FoE} & 51.70 & 0.0159 & 50.60 & 0.0191 & 51.67 & 0.0261 \\
\texttt{NewsLLM}        & 57.81 & 0.1582 & 54.69 & 0.0535 & 58.83 & 0.1608 \\
Improvement     & 11.82\% & 0.1423 & 8.08\% & 0.0344 & 13.86\% & 0.1347 \\
\bottomrule
\end{tabular}
\end{threeparttable}}
\end{table}

==> tables/robustness_study.tex <==
\begin{table*}[t]
    \centering
    \caption{Robustness comparison of \method{} with and without the robust prediction layer (RPL) under deterministic single-modality removal and stochastic modality dropout.
    We report ARR (\%) and SR on AAPL and BTCUSD; higher values indicate better performance.
    For stochastic dropout, each test instance is assigned one modality in advance, and $p$ denotes the probability of zeroing out that assigned modality.}
    \label{tab:robustness_study}
    \small
    \setlength{\tabcolsep}{4.6pt}
    \renewcommand{\arraystretch}{1.12}

    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}lllccccccccc@{}}
        \toprule
        \multirow{2}{*}{\textbf{Metric}}
        & \multirow{2}{*}{\textbf{Asset}}
        & \multirow{2}{*}{\textbf{Method}}
        & \textbf{Clean}
        & \multicolumn{4}{c}{\textbf{Single-Modality Removal}}
        & \multicolumn{4}{c}{\textbf{Stochastic Modality Dropout}} \\
        \cmidrule(lr){4-4}
        \cmidrule(lr){5-8}
        \cmidrule(lr){9-12}
        &
        &
        & Unperturbed
        & Market & Technical & News & Sentiment
        & $p=0.25$ & $p=0.50$ & $p=0.75$ & $p=1.00$ \\
        \midrule

        \multirow{4}{*}{ARR\%$\uparrow$}
        & \multirow{2}{*}{AAPL}
        & \method{}
        & 67.79 & 58.42 & 61.15 & 64.90 & 65.38 & 65.21 & 62.08 & 58.74 & 54.12 \\
        &
        & w/o RPL
        & 62.83 & 51.10 & 54.37 & 58.62 & 59.20 & 58.94 & 54.15 & 48.60 & 42.35 \\

        \cmidrule(lr){2-12}

        & \multirow{2}{*}{BTCUSD}
        & \method{}
        & 84.64 & 72.18 & 76.50 & 81.25 & 82.04 & 81.90 & 78.43 & 73.92 & 68.10 \\
        &
        & w/o RPL
        & 79.81 & 63.45 & 68.20 & 75.10 & 76.32 & 74.88 & 68.25 & 60.18 & 51.40 \\

        \midrule

        \multirow{4}{*}{SR$\uparrow$}
        & \multirow{2}{*}{AAPL}
        & \method{}
        & 1.47 & 1.21 & 1.29 & 1.39 & 1.41 & 1.40 & 1.32 & 1.22 & 1.08 \\
        &
        & w/o RPL
        & 1.29 & 0.98 & 1.06 & 1.18 & 1.20 & 1.19 & 1.07 & 0.92 & 0.76 \\

        \cmidrule(lr){2-12}

        & \multirow{2}{*}{BTCUSD}
        & \method{}
        & 2.65 & 2.18 & 2.34 & 2.52 & 2.55 & 2.54 & 2.40 & 2.22 & 1.98 \\
        &
        & w/o RPL
        & 2.14 & 1.58 & 1.75 & 1.98 & 2.02 & 1.97 & 1.76 & 1.48 & 1.21 \\

        \bottomrule
    \end{tabular}
    }
\end{table*}
